Hyperspectral Imaging and Analysis for Sparse Reconstruction and Recognition

This thesis proposes spatio-spectral techniques for hyperspectral image analysis. Adaptive spatio-spectral support and variable exposure hyperspectral imaging is demonstrated to improve spectral reflectance recovery from hyperspectral images. Novel spectral dimensionality reduction techniques have been proposed from the perspective of spectral only and spatio-spectral information preservation. It was found that the joint sparse and joint group sparse hyperspectral image models achieve lower reconstruction error and higher recognition accuracy using only a small subset of bands. Hyperspectral image databases have been developed and made publicly available for further research in compressed hyperspectral imaging, forensic document analysis and spectral reflectance recovery.

==> contribution.tex <==
\section*{\center \Large Contribution of Candidate to Published Work}

\vspace{5mm}

\noindent My contribution in all the papers was 80\%. I collected the data, developed and implemented the algorithms,
performed the experiments and wrote the papers. My supervisors reviewed the papers and
provided useful feedback for improvement.
